Sparsity Order Estimation from a Single Compressed Observation Vector

We investigate the problem of estimating the unknown degree of sparsity from compressive measurements without the need to carry out a sparse recovery step. While the sparsity order can be directly inferred from the effective rank of the observation matrix in the multiple snapshot case, this appears to be impossible in the more challenging single snapshot case. We show that specially designed measurement matrices allow to rearrange the measurement vector into a matrix such that its effective rank coincides with the effective sparsity order. In fact, we prove that matrices which are composed of a Khatri-Rao product of smaller matrices generate measurements that allow to infer the sparsity order. Moreover, if some samples are used more than once, one of the matrices needs to be Vandermonde. These structural constraints reduce the degrees of freedom in choosing the measurement matrix which may incur in a degradation in the achievable coherence. We thus also address suitable choices of the measurement matrices. In particular, we analyze Khatri-Rao and Vandermonde matrices in terms of their coherence and provide a new design for Vandermonde matrices that achieves a low coherence.

==> snippets/tex/poster_skel/head.tex <==
\usepackage{psfrag}
\usepackage{array,makecell,booktabs}
\usepackage{filecontents}
\usepackage{longtable,tabularx}
\usepackage[size=a0,width=90,height=120,scale=1.4,orientation=portrait]{beamerposter}
\setbeamertemplate{navigation symbols}{}
\usepackage{tabularx}
\usepackage[none]{hyphenat}
\usepackage{bm}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{comment}
%\usepackage{natbib}
\usepackage{epstopdf}
\usepackage{booktabs}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{amsfonts, amsmath, amsthm, amssymb}
\usepackage{wrapfig}
\usepackage{wasysym}
\usepackage[justification=centering]{caption}
\usepackage[english]{babel}

\usepackage{tikz}
\usepackage{graphicx}
\usetikzlibrary{matrix,arrows,shapes,trees,fit}
\usetikzlibrary{calc,positioning,scopes,backgrounds}
\newif\ifoutertikznest
\outertikznestfalse
\usetikzlibrary{decorations.markings}

\newcommand{\tikzwidth}{0.48\textwidth}
\tikzstyle{lw} = [line width=3pt]

\usepackage{pgfplots}
\pgfplotsset{compat=newest}

\definecolor{box_white}{cmyk}{0.0361,0.0251,0.0166,0}
\definecolor{text_black}{cmyk}{0.7979,0.7417,0.6916,0.6554}
\definecolor{tui_orange_dark}{cmyk}{0,0.6,1,0} 
\definecolor{tui_orange_light}{cmyk}{0.0000,0.0876, 0.1474, 0.0157}
\definecolor{tui_green_dark}{cmyk}{1,0,0.5,0.2}
\definecolor{tui_green_light}{cmyk}{0.0576,0.0041, 0.0000, 0.0471} 
\definecolor{tui_blue_dark}{cmyk}{1.0000,0.5000,0.0000,0.6000}
\definecolor{tui_blue_light}{cmyk}{0.0920,0.0440,0.0000,0.0196}
\definecolor{tui_red_dark}{cmyk}{0.0000,1.0000,1.0000,0.2000}
\definecolor{tui_red_light}{cmyk}{0.0000,0.1107,0.1107,0.0078}

\pgfplotscreateplotcyclelist{tui_dark}{
{tui_orange_dark,mark=*},
{tui_green_dark,mark=square},
{tui_blue_dark,mark=triangle},
{tui_red_dark,mark=diamond},
}

\pgfplotsset{
    cycle list name=tui_dark,
}


\setbeamercolor{itemize item}{fg=tui_red_dark,bg=white}
\setbeamercolor{headline}{fg=black,bg=tui_blue_dark}
\setbeamercolor{title in headline}{fg=white}
\setbeamercolor{author in headline}{fg=white}
\setbeamercolor{institute in headline}{fg=white}
\setbeamercolor{logo in headline}{fg=black,bg=lightgray}
\setbeamercolor{footline}{fg=white,bg=tui_blue_dark}
\setbeamercolor{block}{fg=white,bg=umic_bg}
\setbeamercolor{caption name}{fg=tui_blue_dark}
\setbeamerfont{caption}{size=\small}

\setbeamercolor*{block body}{fg=text_black,bg=box_white}
\setbeamercolor*{block title}{fg=white,bg=tui_orange_dark}
\setbeamerfont{block title}{size=\normalsize,series=\bf}
\setbeamerfont{block body}{size=\normalsize}
\setbeamercolor{footlinecolor}{fg=white,bg=tui_blue_dark}
\setbeamertemplate{caption}[numbered]

%
% includes a logo wrapped around its own column
% scaling and path have to specified
%
\newcommand{\addlogo}[2]{
\begin{column}{.2\paperwidth}
\begin{center}
\topskip0pt
\vspace*{\fill}
\includegraphics[scale = #2]{#1}
\vspace*{\fill}
\end{center}
\end{column}
}

%
% put a light green frame around 
% something important within a text box
%
\newcommand{\frameIt}[2]{
	\begin{center}
	\vspace{13mm}
	\setbeamercolor*{block title}{fg=text_black,bg=tui_green_light}
	\setbeamercolor*{block body}{fg=text_black,bg=tui_green_light}
	\begin{minipage}{0.85\textwidth}
	\begin{block}{#1}\vspace{-8mm}\centering#2
	\end{block}
	\end{minipage}
	\end{center}
	\vspace{-10mm}
}
